Are We Ready to Embrace Generative AI for Software Q&A?

Stack Overflow, the world's largest software Q&A (SQA) website, is facing a significant traffic drop due to the emergence of generative AI techniques. ChatGPT is banned by Stack Overflow after only 6 days from its release. The main reason provided by the official Stack Overflow is that the answers generated by ChatGPT are of low quality. To verify this, we conduct a comparative evaluation of human-written and ChatGPT-generated answers. Our methodology employs both automatic comparison and a manual study. Our results suggest that human-written and ChatGPT-generated answers are semantically similar, however, human-written answers outperform ChatGPT-generated ones consistently across multiple aspects, specifically by 10% on the overall score. We release the data, analysis scripts, and detailed results at https://anonymous.4open.science/r/GAI4SQA-FD5C.

==> 6_Lessons_learned.tex <==
% \noindent\textbf{\gpt{} tends to be conservative in answering different questions differently}. We find that the human-written answers are averagely longer than \gpt{}-generated answers but ChatGPT generates more answers that are longer than the human-written ones. It implies that human is more daring to provide answers with a wide range of length accordingly while \gpt{} is more likely to generate answers with similar length for different questions.



\noindent\textbf{Interactive SQA may lead to better answers}. We find that after a question is created on \so{}, it takes more than 13 days (19,840 minutes) on average to receive a high-quality answer that can be accepted. With the help of \gpt{}, a desired answer can be immediately generated, and based on our result, the average overall score of \gpt{}-generated answers is 3.65. In other words, the quality of the answers is close to the human-satisfied level.
Thus, leveraging \gpt{}-like techniques to generate an initial version of the answer and then involve humans in the loop to iteratively improve the answer by interacting with AI may be a promising future direction to explore for SQA.

% \noindent\textbf{Leverage \gpt{} to answer questions with code}. Based on our result, we find that humans and \gpt{} have low agreement on whether a question needs to be answered with code. Thus, we advocate future research on determining a question that needs to be answered with code. Moreover, we find that \gpt{} tends to provide code more than humans. Intuitively, providing a solution with code examples is preferable rather than simply explaining due to the nature of software technical problems.
% And considering the strong code generation and synthesis capability of \gpt{}-like techniques demonstrated by many prior works~\cite{xia2023automated}, we point out that such capability may have a big potential to enhance human answers.


==> Background.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[ht]
\begin{tabular}{l|p{15cm}} \hline
Question Link  & \url{https://stackoverflow.com/questions/71641264} \\ \hline
Question Title & How can I solve this issue on Mac M1 Caused by: java.lang.Exception: No native library is found for os.name=Mac and os.arch=aarch64       \\ \hline
Question Body  & \begin{tabular}[c]{@{}p{15cm}@{}}I solved this issue with the code below in my build.gradle\\ \\ {[}Code{]}\\ \\ But it has an effect on the project I am working on. for some reason, it is not working with room sql implemented on the project.\\ I get this error when i removed the code above.\\ Is there a better approach to solve this.\\ \\ {[}Error Message{]}\end{tabular}     \\ \hline
Human Answer   & \begin{tabular}[c]{@{}p{15cm}@{}}update your room library\\ \\ {[}Code{]} \\ \\ Here is Reference.\end{tabular}      \\ \hline
ChatGPT Answer & \begin{tabular}[c]{@{}p{15cm}@{}}The issue seems to be related to the lack of native support of SQLite for the M1 chip architecture. The code you provided is a workaround that forces the usage of a specific SQLite version that might work on your system. However, this is not recommended as it can cause issues with other dependencies that rely on different versions of SQLite. \\ \\ A better approach to solving this issue would be to wait for the SQLite team to provide native support for the M1 chip architecture. In the meantime, you can try running your project through Rosetta emulation, which should allow it to use the existing SQLite library. \\ \\ Another potential workaround is to use a different database engine that supports the M1 chip architecture, such as PostgreSQL or MySQL.\end{tabular}\\ \hline
\end{tabular}%
\caption{}
\label{tab:my-table}
\end{table*}




==> Data.tex <==



